Addressing Fairness, Bias and Class Imbalance in Machine Learning: the FBI-loss

Resilience to class imbalance and confounding biases, together with the assurance of fairness guarantees are highly desirable properties of autonomous decision-making systems with real-life impact. Many different targeted solutions have been proposed to address separately these three problems, however a unifying perspective seems to be missing. With this work, we provide a general formalization, showing that they are different expressions of unbalance. Following this intuition, we formulate a unified loss correction to address issues related to Fairness, Biases and Imbalances (FBI-loss). The correction capabilities of the proposed approach are assessed on three real-world benchmarks, each associated to one of the issues under consideration, and on a family of synthetic data in order to better investigate the effectiveness of our loss on tasks with different complexities. The empirical results highlight that the flexible formulation of the FBI-loss leads also to competitive performances with respect to literature solutions specialised for the single problems.

==> Declaration.tex <==
\section*{Declaration}
According to guidelines at https://www.springer.com/journal/10994/submission-guidelines

\subsection*{Funding}
The work by Davide Bacciu is partially supported by TAILOR, a project funded by EU Horizon 2020 research and innovation programme under GA No 952215.

\subsection*{Conflict of interest}
There are no conflicts of interest to disclose

\subsection*{Availability of data and material}
All real data are publicly available at the locations found in the references. Simulated data are extensively described so as to be reproducible. They can also be made available on request.

\subsection*{Code availability}
The code is available at \url{https://bitbucket.org/elisaferrari/fbi-loss-code.git}.

\subsection*{Authors contributions}
Conceptualization: Elisa Ferrari, Davide Bacciu; Methodology: Elisa Ferrari; Formal analysis and investigation: Elisa Ferrari; Writing - original draft preparation: Elisa Ferrari; Writing - review and editing: Davide Bacciu; Supervision: Davide Bacciu.

